A Latent Mixture Model for Heterogeneous Causal Mechanisms in Mendelian Randomization

Mendelian Randomization (MR) is a popular method in epidemiology and genetics that uses genetic variation as instrumental variables for causal inference. Existing MR methods usually assume most genetic variants are valid instrumental variables that identify a common causal effect. There is a general lack of awareness that this effect homogeneity assumption can be violated when there are multiple causal pathways involved, even if all the instrumental variables are valid. In this article, we introduce a latent mixture model MR-PATH that groups instruments that yield similar causal effect estimates together. We develop a Monte-Carlo EM algorithm to fit this mixture model, derive approximate confidence intervals for uncertainty quantification, and adopt a modified Bayesian Information Criterion (BIC) for model selection. We verify the efficacy of the Monte-Carlo EM algorithm, confidence intervals, and model selection criterion using numerical simulations. We identify potential mechanistic heterogeneity when applying our method to estimate the effect of high-density lipoprotein cholesterol on coronary heart disease and the effect of adiposity on type II diabetes.

==> tikz/dag_mult_mech.tex <==
\tikzset{SNP/.style = {draw, circle, minimum size=1.5cm}}
\tikzset{M/.style = {draw, circle, minimum height=1.5cm, minimum width=1.5cm}}
\tikzset{Xcomp/.style={draw, circle, minimum height=1.7cm, minimum width=1.7cm}}
\tikzset{>=latex, shorten >=.5pt}

% \tikzset{
%     pics/SNPset/.style n args={3}{
%         code = { %
%             \node[SNP, #1] (Z1) at (0,0) {#2};
%             \node[SNP, #1, below=.5cm of Z1] (Zj) {#3};
%             \node[#1] (dots) at ($(Z1)!.4!(Zj)$) {\vdots};
%         }
%     }
% }

\begin{figure}
 \begin{subfigure}[t]{.47\linewidth}
  \centering
  \begin{tikzpicture}[every node/.style={scale=0.6}]  \Large
   \def \firstcolor {red}
   \def \secondcolor {blue}
   \def \thirdcolor {violet}

   \node[SNP, \firstcolor] (Z1-1) {$Z_{1,1}$};
   \node[\firstcolor, below of=Z1-1] (dots1) {\vdots};
   \node[SNP, \firstcolor, below=.1cm of dots1.south] (Z1-p) {$Z_{1,p_1}$};

   \node[SNP, \secondcolor, below=.5cm of Z1-p] (Z2-1) {$Z_{2,1}$};
   \node[\secondcolor, below of=Z2-1] (dots2) {\vdots};
   \node[SNP, \secondcolor, below=.1cm of dots2] (Z2-p) {$Z_{2,p_2}$};

   \node[SNP, \thirdcolor, below=.5cm of Z2-p] (Z3-1) {$Z_{3,1}$};
   \node[\thirdcolor, below of=Z3-1] (dots3) {\vdots};
   \node[SNP, \thirdcolor, below=.1cm of dots3] (Z3-p) {$Z_{3,p_3}$};

   \node[M, \firstcolor, right=1.2cm of dots1] (M1) {$M_1$};
   % \draw[->, \firstcolor, shorten <=0.5cm] (dots1) to (M1);
   \draw[->, \firstcolor] (Z1-1) to (M1);
   \draw[->, \firstcolor] (Z1-p) to (M1);

   \node[M, \secondcolor, right=1.2cm of dots2] (M2) {$M_2$};
   % \draw[->, \firstcolor, shorten <=0.5cm] (dots1) to (M1);
   \draw[->, \secondcolor] (Z2-1) to (M2);
   \draw[->, \secondcolor] (Z2-p) to (M2);

   \node[M, \thirdcolor, right=1.2cm of dots3] (M3) {$M_3$};
   % \draw[->, \firstcolor, shorten <=0.5cm] (dots1) to (M1);
   \draw[->, \thirdcolor] (Z3-1) to (M3);
   \draw[->, \thirdcolor] (Z3-p) to (M3);

   \node[draw, circle, minimum height=1.7cm, minimum width=1.7cm, right=1.5cm of M2] (X) {$X$};
   \draw[->, \firstcolor] (M1) to node[above] {$\theta_1$} (X);
   \draw[->, \secondcolor] (M2) to node[above] {$\theta_2$} (X);
   \draw[->, \thirdcolor] (M3) to node[above] {$\theta_3$} (X);

   \node[draw, circle, minimum height=1.7cm, minimum width=1.7cm, right=2 of X] (Y) {$Y$};
   \draw[->] (X) to node[above] {$\beta$} (Y);
   \draw[->, \secondcolor,  bend right] (M2) to node[below] {$\alpha_2$} (Y);
   \draw[->, \thirdcolor, bend right] (M3) to node[above]
   {$\alpha_3$} (Y);

   \node[draw, circle, minimum height=1.7cm, minimum
    width=1.7cm, above right=1cm of X] (U) {$U$};
   \draw[->] (U) to (X);
   \draw[->] (U) to (Y);
  \end{tikzpicture}
  \caption{Scenario 1: Multiple pathways of horizontal pleiotropy.}
  \label{fig:multiple-direct-effect}
 \end{subfigure} %
 \hspace{25pt}
 \begin{subfigure}[t]{.47\linewidth}
  \centering
  \begin{tikzpicture}[every node/.style={scale=0.6}] \Large
   \def \firstcolor {red}
   \def \secondcolor {blue}
   \def \thirdcolor {violet}

   \node[SNP, \firstcolor] (Z1) {$Z_{1,1}$};
   \node[\firstcolor, below of=Z1] (dots1) {\vdots};
   \node[SNP, \firstcolor, below=.1cm of dots1.south] (Zj) {$Z_{1,p_1}$};

   \node[M, \firstcolor, right=1.2cm of dots1] (M1) {$M_1$};
   % \draw[->, \firstcolor, shorten <=0.5cm] (dots1) to (M1);
   \draw[->, \firstcolor] (Z1) to (M1);
   \draw[->, \firstcolor] (Zj) to (M1);

   \node[Xcomp, \firstcolor, right=1cm of M1] (X1) {$X_1$};
   \draw[->, \firstcolor] (M1) to node[above] {$\theta_1$} (X1);


   \node[SNP, \secondcolor, below=.5cm of Zj] (Zj1) {$Z_{2,1}$};
   \node[\secondcolor, below of=Zj1] (dots2) {\vdots};
   \node[SNP, \secondcolor, below=.1cm of dots2] (Zp) {$Z_{2,p_2}$};

   \node[M, \secondcolor, right=1.2cm of dots2] (M2) {$M_2$};
   \draw[->, \secondcolor] (Zj1) to (M2);
   \draw[->, \secondcolor] (Zp) to (M2);

   \node[Xcomp, \secondcolor, right=1cm of M2] (X2) {$X_2$};
   \draw[->, \secondcolor] (M2) to node[above] {$\theta_2$} (X2);

   \node[SNP, \thirdcolor, below=.5cm of Z2-p] (Z3-1) {$Z_{3,1}$};
   \node[\thirdcolor, below of=Z3-1] (dots3) {\vdots};
   \node[SNP, \thirdcolor, below=.1cm of dots3] (Z3-p) {$Z_{3,p_3}$};

   \node[M, \thirdcolor, right=1.2cm of dots3] (M3) {$M_3$};
   % \draw[->, \firstcolor, shorten <=0.5cm] (dots1) to (M1);
   \draw[->, \thirdcolor] (Z3-1) to (M3);
   \draw[->, \thirdcolor] (Z3-p) to (M3);

   \node[Xcomp, \thirdcolor, right=1cm of M3] (X3) {$X_3$};
   \draw[->, \thirdcolor] (M3) to node[above] {$\theta_3$} (X3);

   \node[draw, rectangle, minimum height=12.5cm, minimum
    width=2.7cm] (X) at ($(X1)!.5!(X3)$) {};
   \node[below=.1cm of X.south] {\large $X = X_1 + X_2 + X_3$};

   \node[draw, circle, minimum height=1.7cm, minimum width=1.7cm, right=1.5cm of X2] (Y) {$Y$};
   \draw[->, \firstcolor] (X1) to node[above] {$\beta_1$} (Y);
   \draw[->, \secondcolor] (X2) to node[above] {$\beta_2$} (Y);
   \draw[->, \thirdcolor] (X3) to node[above] {$\beta_3$}
   (Y);

   \node[draw, circle, minimum height=1.7cm, minimum  width=1.7cm, above=1.5cm of Y] (U) {$U$};
   \draw[->] (U) to (X1);
   \draw[->] (U) to (X2);
   \draw[->] (U) to (X3);
   \draw[->] (U) to (Y);

  \end{tikzpicture}
  \caption{Scenario 2: Multiple mechanisms for the exposure $X$.}
  \label{fig:multiple-x}
 \end{subfigure}
 \caption{Two scenarios of mechanistic heterogeneity.}
 \label{fig:mechanistic-heterogeneity}
\end{figure}





%%%%%%%%%% Old drawing
% \begin{figure}
%   \centering
%   \begin{tikzpicture}
%     \node[rectangle, draw, minimum height=4cm, minimum width=2.3cm] (X) at (0, -0.1) {};
%     \node[above of=X,yshift=36] (X-text) {$X$ (Exposure)};
%     \node[rectangle, draw, minimum width=2cm, minimum height=0.8cm, violet] (X1) at (0,0.7) {};
%     \node[rectangle, draw, minimum width=2cm, minimum height=0.8cm, blue] (X2) at (0,-0.8) {};
%     \node[rectangle, draw] (Y) at (4.5, 0) {$Y$ (Outcome)};

%     \node[rectangle, draw, violet] (Z1) at (-5, 1.5) {$Z_1$ (SNP \#$1$)};
%     \node[purple] (dots1) at (-5, 1) {$\vdots$} {};
%     \node[rectangle, draw, violet] (Zj) at (-5, 0.3) {$Z_{p_1}$ (SNP \#$p_1$)};

%     \node[rectangle, draw, violet, minimum height=0.9cm, minimum width = 0.9cm] (M1) at (-2.2, 0.7) {$M_1$};

%     \node[rectangle, draw, blue] (Zj1) at (-3.8, -0.5) {$Z_{i+1}$ (SNP \#$i$+$1$)};
%     \node[rectangle, draw, blue] (Zp) at (-3.5, -1.7) {$Z_p$ (SNP \#$p$)};
%     \node[blue] (dots2) at (-3.5, -1) {$\vdots$} {};
%     \draw[->, violet] (X1) -- (Y);
%     \draw[->, blue] (X2) -- (Y);
%     % \draw[->] (U) to (Y);
%     % \draw[->] (U) to (X);
%     \draw[->, violet] (Z1) -- (M1);
%     \draw[->, violet] (Zj) -- (M1);
%     \draw[->, violet] (M1) -- (X1);
%     \draw[->, blue] (Zj1) -- (X2);
%     \draw[->, blue] (Zp) -- (X2);
%     % \node[below of=X, yshift=-40] (subtraits) {\small HDL subtraits};
%     % \draw[->, shorten >= 4pt] (subtraits) -- (X);
%   \end{tikzpicture}
%   \caption{}
%   \label{fig:dag-mult-mech}
% \end{figure}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes.geometric}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
% \tikzstyle{const} = [rectangle, inner sep=3pt, node distance=1]
\tikzstyle{const} = [regular polygon, regular polygon sides=4, draw=black, inner
sep=1pt, fill=gray!100]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

